The Non-Linear Power Spectrum of the Lyman Alpha Forest

The Lyman alpha forest power spectrum has been measured on large scales by the BOSS survey in SDSS-III at $z\sim 2.3$, has been shown to agree well with linear theory predictions, and has provided the first measurement of Baryon Acoustic Oscillations at this redshift. However, the power at small scales, affected by non-linearities, has not been well examined so far. We present results from a variety of hydrodynamic simulations to predict the redshift space non-linear power spectrum of the Lyman Alpha transmission for several models, testing the dependence on resolution and box size. A new fitting formula is introduced to facilitate the comparison of our simulation results with observations and other simulations. The non-linear power spectrum has a generic shape determined by a transition scale from linear to non-linear anisotropy, and a Jeans scale below which the power drops rapidly. In addition, we predict the two linear bias factors of the Lyman Alpha forest and provide a better physical interpretation of their values and redshift evolution. The dependence of these bias factors and the non-linear power on the amplitude and slope of the primordial fluctuations power spectrum, the temperature-density relation of the intergalactic medium, and the mean Lyman Alpha transmission, as well as the redshift evolution, is investigated and discussed in detail. A preliminary comparison to the observations shows that the predicted redshift distortion parameter is in good agreement with the recent determination of Blomqvist et al., but the density bias factor is lower than observed. We make all our results publicly available in the form of tables of the non-linear power spectrum that is directly obtained from all our simulations, and parameters of our fitting formula.

==> tables/Fvar_planck_table.tex <==
\begin{table}[!htbp]
 \centering
 \caption{Values of the bias parameters for different mean transmision fraction renormalization on the Planck simulation. 
  \vspace{2 mm}}{ 
  \begin{tabular}{c|*{3}c}
 z  & $\beta$    & $b_{\tau\delta}$  &  $b_{\tau\eta}$ \\ 
  \hline 
  \hline 
  \multicolumn{4}{l}{$\bar{F} = $0.775} \\ 
 \hline 
2.4  & $1.37  \pm  0.064$  & $0.683  \pm  0.012$  & $0.967  \pm  0.045$ \\
2.2  & $1.42  \pm  0.071$  & $0.778  \pm  0.013$  & $1.14  \pm  0.056$ \\
\hline 
\multicolumn{4}{l}{$\bar{F} = $0.80} \\ 
 \hline 
2.4  & $1.39  \pm  0.058$  & $0.573  \pm  0.0085$  & $0.822  \pm  0.034$ \\
2.2  & $1.43  \pm  0.06$  & $0.517  \pm  0.0075$  & $0.766  \pm  0.032$ \\
\hline 
\multicolumn{4}{l}{$\bar{F} = $0.825} \\ 
 \hline 
2.4  & $1.39  \pm  0.052$  & $0.6  \pm  0.0088$  & $0.858  \pm  0.032$ \\
2.2  & $1.43  \pm  0.056$  & $0.547  \pm  0.0079$  & $0.81  \pm  0.032$ \\
\hline 
\multicolumn{4}{l}{$\bar{F} = $0.8518} \\ 
 \hline 
2.4  & $1.38  \pm  0.05$  & $0.638  \pm  0.0086$  & $0.909  \pm  0.033$ \\
2.2  & $1.42  \pm  0.05$  & $0.581  \pm  0.0078$  & $0.857  \pm  0.03$ \\
\hline 
  \end{tabular}
 }
 \end{table}


\begin{table}[!htbp]
\centering
 \caption{Values of the fitting parameters for different mean transmision fraction renormalization on the Planck simulation .
  \vspace{2 mm}}
 \adjustbox{width=1.05 \textwidth}{ 
  \begin{tabular}{c|*{6}c}
 z  &  $q_{1}$  &  $k_p\,[h/Mpc]$ &  $k_{v}^{a_v}\,[h/Mpc]^{a_v}$  &  $a_v$  &  $b_v$ &  $k_{na}$ \\ 
  \hline 
  \hline 
  \multicolumn{7}{l}{$\bar{F} = $0.775} \\ 
 \hline 
2.4  & $0.779  \pm  0.043$  & $16.9  \pm  1.1$  & $0.95  \pm  0.094$  & $0.516  \pm  0.032$  & $1.61  \pm  0.024$  & $3.41  \pm  0.05$ \\
2.2  & $0.734  \pm  0.038$  & $15.4  \pm  0.83$  & $0.865  \pm  0.08$  & $0.459  \pm  0.031$  & $1.59  \pm  0.025$  & $3.19  \pm  0.049$ \\
\hline 
\multicolumn{7}{l}{$\bar{F} = $0.80} \\ 
 \hline 
2.4  & $0.796  \pm  0.04$  & $18.8  \pm  1.3$  & $0.982  \pm  0.087$  & $0.535  \pm  0.03$  & $1.62  \pm  0.011$  & $3.02  \pm  0.031$ \\
2.2  & $0.77  \pm  0.035$  & $16.4  \pm  0.83$  & $0.92  \pm  0.073$  & $0.478  \pm  0.027$  & $1.59  \pm  0.012$  & $2.82  \pm  0.034$ \\
\hline 
\multicolumn{7}{l}{$\bar{F} = $0.825} \\ 
 \hline 
2.4  & $0.862  \pm  0.039$  & $20.1  \pm  1.6$  & $1.08  \pm  0.086$  & $0.554  \pm  0.027$  & $1.61  \pm  0.011$  & $3  \pm  0.023$ \\
2.2  & $0.812  \pm  0.035$  & $17.7  \pm  1.1$  & $0.984  \pm  0.076$  & $0.497  \pm  0.026$  & $1.6  \pm  0.0098$  & $2.81  \pm  0.026$ \\
\hline 
\multicolumn{7}{l}{$\bar{F} = $0.8518} \\ 
 \hline 
2.4  & $0.921  \pm  0.037$  & $22.9  \pm  2.3$  & $1.16  \pm  0.09$  & $0.571  \pm  0.028$  & $1.62  \pm  0.0086$  & $2.96  \pm  0.025$ \\
2.2  & $0.866  \pm  0.033$  & $19.4  \pm  1.5$  & $1.06  \pm  0.075$  & $0.514  \pm  0.025$  & $1.6  \pm  0.0091$  & $2.77  \pm  0.023$ \\
\hline 
  \end{tabular}
 }
 \end{table}


==> tables/table_F0_apm7_bias.tex <==
\begin{table}[!htbp]
 \adjustbox{width=1.2 \textwidth}{ 
  \begin{tabular}{c|*{3}c}
 z  & $\beta$  &  $b_{\tau\delta}$  & $b_{\tau\eta}$   \\ 
  \hline 
  \hline 
  \multicolumn{4}{l}{F0775} \\ 
 \hline 
2.4  & $1.37  \pm  0.064$  & $0.683  \pm  0.012$  & $0.967  \pm  0.045$ \\
2.2  & $1.42  \pm  0.071$  & $0.778  \pm  0.013$  & $1.14  \pm  0.056$ \\
\hline 
\multicolumn{4}{l}{F08} \\ 
 \hline 
2.4  & $1.39  \pm  0.058$  & $0.573  \pm  0.0085$  & $0.822  \pm  0.034$ \\
2.2  & $1.43  \pm  0.06$  & $0.517  \pm  0.0075$  & $0.766  \pm  0.032$ \\
\hline 
\multicolumn{4}{l}{F0825} \\ 
 \hline 
2.4  & $1.39  \pm  0.052$  & $0.6  \pm  0.0088$  & $0.858  \pm  0.032$ \\
2.2  & $1.43  \pm  0.056$  & $0.547  \pm  0.0079$  & $0.81  \pm  0.032$ \\
\hline 
\multicolumn{4}{l}{F0852} \\ 
 \hline 
2.4  & $1.38  \pm  0.05$  & $0.638  \pm  0.0086$  & $0.909  \pm  0.033$ \\
2.2  & $1.42  \pm  0.05$  & $0.581  \pm  0.0078$  & $0.857  \pm  0.03$ \\
\hline 


==> tables/table_F0_apm7_par.tex <==
\begin{table}[!htbp]
 \adjustbox{width=1.2 \textwidth}{ 
  \begin{tabular}{c|*{6}c}
 z  &  $q_{1}$  &  $k_p\,[h/Mpc]$ &  $k_{v}^{a_v}\,[h/Mpc]^{a_v}$  &  $a_v$  &  $b_v$ &  $k_{\mu}$ \\ 
  \hline 
  \hline 
  \multicolumn{7}{l}{F0775} \\ 
 \hline 
2.4  & $0.779  \pm  0.043$  & $16.9  \pm  1.1$  & $0.95  \pm  0.094$  & $0.516  \pm  0.032$  & $1.61  \pm  0.024$  & $3.41  \pm  0.05$ \\
2.2  & $0.734  \pm  0.038$  & $15.4  \pm  0.83$  & $0.865  \pm  0.08$  & $0.459  \pm  0.031$  & $1.59  \pm  0.025$  & $3.19  \pm  0.049$ \\
\hline 
\multicolumn{7}{l}{F08} \\ 
 \hline 
2.4  & $0.796  \pm  0.04$  & $18.8  \pm  1.3$  & $0.982  \pm  0.087$  & $0.535  \pm  0.03$  & $1.62  \pm  0.011$  & $3.02  \pm  0.031$ \\
2.2  & $0.77  \pm  0.035$  & $16.4  \pm  0.83$  & $0.92  \pm  0.073$  & $0.478  \pm  0.027$  & $1.59  \pm  0.012$  & $2.82  \pm  0.034$ \\
\hline 
\multicolumn{7}{l}{F0825} \\ 
 \hline 
2.4  & $0.862  \pm  0.039$  & $20.1  \pm  1.6$  & $1.08  \pm  0.086$  & $0.554  \pm  0.027$  & $1.61  \pm  0.011$  & $3  \pm  0.023$ \\
2.2  & $0.812  \pm  0.035$  & $17.7  \pm  1.1$  & $0.984  \pm  0.076$  & $0.497  \pm  0.026$  & $1.6  \pm  0.0098$  & $2.81  \pm  0.026$ \\
\hline 
\multicolumn{7}{l}{F0852} \\ 
 \hline 
2.4  & $0.921  \pm  0.037$  & $22.9  \pm  2.3$  & $1.16  \pm  0.09$  & $0.571  \pm  0.028$  & $1.62  \pm  0.0086$  & $2.96  \pm  0.025$ \\
2.2  & $0.866  \pm  0.033$  & $19.4  \pm  1.5$  & $1.06  \pm  0.075$  & $0.514  \pm  0.025$  & $1.6  \pm  0.0091$  & $2.77  \pm  0.023$ \\
\hline 
  \end{tabular}
 }
 \end{table}
 

==> tables/table_Planck_qpm8_bias.tex <==
\begin{table}[!htbp]
 \adjustbox{width=1.2 \textwidth}{ 
  \begin{tabular}{c|*{3}c}
 z  & $\beta  &  $b_{\tau\delta}$ & $b_{\tau\eta}$ \\ 
  \hline 
  \hline 
  \multicolumn{4}{l}{Planck} \\ 
 \hline 
3.0  & $1.07  \pm  0.0592$  & $0.646  \pm  0.0185$  & $0.657  \pm  0.0454$ \\
2.8  & $1.16  \pm  0.0649$  & $0.657  \pm  0.0167$  & $0.723  \pm  0.0492$ \\
2.6  & $1.25  \pm  0.044$  & $0.66  \pm  0.0109$  & $0.791  \pm  0.0336$ \\
2.4  & $1.29  \pm  0.0736$  & $0.678  \pm  0.0154$  & $0.84  \pm  0.056$ \\
2.2  & $1.32  \pm  0.0569$  & $0.675  \pm  0.0141$  & $0.858  \pm  0.0442$ \\
\hline 
\multicolumn{4}{l}{Planck} \\ 
 \hline 
3.0  & $1.07  \pm  0.0592$  & $0.646  \pm  0.0185$  & $0.657  \pm  0.0454$ \\
2.8  & $1.16  \pm  0.0649$  & $0.657  \pm  0.0167$  & $0.723  \pm  0.0492$ \\
2.6  & $1.25  \pm  0.044$  & $0.66  \pm  0.0109$  & $0.791  \pm  0.0336$ \\
2.4  & $1.29  \pm  0.0736$  & $0.678  \pm  0.0154$  & $0.84  \pm  0.056$ \\
2.2  & $1.32  \pm  0.0569$  & $0.675  \pm  0.0141$  & $0.858  \pm  0.0442$ \\
\hline 


==> tables/table_Planck_qpm8_par.tex <==
\begin{table}[!htbp]
 \adjustbox{width=1.2 \textwidth}{ 
  \begin{tabular}{c|*{6}c}
 z  &  $q_1$ & $q_2$  &  $k_p$  &  $k_v$  &  $a_v$  &  $b_v$ \\ 
  \hline 
  \hline 
  \multicolumn{7}{l}{Planck} \\ 
 \hline 
3.0  & $0.000377  \pm  0.224$  & $0.787  \pm  0.22$  & $11.8  \pm  1.17$  & $0.552  \pm  0.201$  & $0.178  \pm  0.108$  & $1.64  \pm  0.0253$ \\
2.8  & $-0.0168  \pm  0.169$  & $0.711  \pm  0.143$  & $12  \pm  0.963$  & $0.548  \pm  0.126$  & $0.203  \pm  0.0725$  & $1.65  \pm  0.028$ \\
2.6  & $0.000363  \pm  0.124$  & $0.651  \pm  0.113$  & $11.8  \pm  0.977$  & $0.545  \pm  0.115$  & $0.195  \pm  0.0729$  & $1.64  \pm  0.0168$ \\
2.4  & $-0.00197  \pm  0.111$  & $0.623  \pm  0.0688$  & $10.9  \pm  0.463$  & $0.517  \pm  0.0275$  & $0.152  \pm  0.0347$  & $1.62  \pm  0.0175$ \\
2.2  & $0.0405  \pm  0.089$  & $0.534  \pm  0.0485$  & $10.6  \pm  0.343$  & $0.534  \pm  0.0217$  & $0.139  \pm  0.029$  & $1.6  \pm  0.0146$ \\
\hline 
\multicolumn{7}{l}{Planck} \\ 
 \hline 
3.0  & $0.000377  \pm  0.224$  & $0.787  \pm  0.22$  & $11.8  \pm  1.17$  & $0.552  \pm  0.201$  & $0.178  \pm  0.108$  & $1.64  \pm  0.0253$ \\
2.8  & $-0.0168  \pm  0.169$  & $0.711  \pm  0.143$  & $12  \pm  0.963$  & $0.548  \pm  0.126$  & $0.203  \pm  0.0725$  & $1.65  \pm  0.028$ \\
2.6  & $0.000363  \pm  0.124$  & $0.651  \pm  0.113$  & $11.8  \pm  0.977$  & $0.545  \pm  0.115$  & $0.195  \pm  0.0729$  & $1.64  \pm  0.0168$ \\
2.4  & $-0.00197  \pm  0.111$  & $0.623  \pm  0.0688$  & $10.9  \pm  0.463$  & $0.517  \pm  0.0275$  & $0.152  \pm  0.0347$  & $1.62  \pm  0.0175$ \\
2.2  & $0.0405  \pm  0.089$  & $0.534  \pm  0.0485$  & $10.6  \pm  0.343$  & $0.534  \pm  0.0217$  & $0.139  \pm  0.029$  & $1.6  \pm  0.0146$ \\
\hline 
  \end{tabular}
 }
 \end{table}
 

==> tables/table_Q2lliure_qpm8_bias.tex <==
\begin{table}[!htbp]
 \adjustbox{width=1.2 \textwidth}{ 
  \begin{tabular}{c|*{3}c}
 z  & $\beta  &  $b_{\tau\delta}$ & $b_{\tau\eta}$ \\ 
  \hline 
  \hline 
  \multicolumn{4}{l}{Fiducial} \\ 
 \hline 
3.0  & $ 1.179  \pm   0.061$  & $0.6010  \pm  0.0126$  & $ 0.722  \pm   0.039$ \\
2.8  & $ 1.256  \pm   0.049$  & $0.6096  \pm  0.0132$  & $ 0.784  \pm   0.033$ \\
2.6  & $ 1.292  \pm   0.069$  & $0.6206  \pm  0.0146$  & $ 0.823  \pm   0.046$ \\
2.4  & $ 1.321  \pm   0.067$  & $0.6286  \pm  0.0130$  & $ 0.856  \pm   0.044$ \\
2.2  & $ 1.347  \pm   0.047$  & $0.6306  \pm  0.0099$  & $ 0.882  \pm   0.031$ \\
\hline 
\multicolumn{4}{l}{R384C} \\ 
 \hline 
3.0  & $ 1.200  \pm   0.067$  & $0.5981  \pm  0.0194$  & $ 0.732  \pm   0.045$ \\
2.8  & $ 1.288  \pm   0.068$  & $0.6043  \pm  0.0137$  & $ 0.797  \pm   0.044$ \\
2.6  & $ 1.355  \pm   0.070$  & $0.6096  \pm  0.0116$  & $ 0.848  \pm   0.044$ \\
2.4  & $ 1.399  \pm   0.078$  & $0.6147  \pm  0.0144$  & $ 0.887  \pm   0.050$ \\
2.2  & $ 1.426  \pm   0.074$  & $0.6144  \pm  0.0126$  & $ 0.909  \pm   0.047$ \\
\hline 
\multicolumn{4}{l}{L120} \\ 
 \hline 
3.0  & $ 1.204  \pm   0.032$  & $0.5808  \pm  0.0978$  & $ 0.713  \pm   0.117$ \\
2.8  & $ 1.296  \pm   0.028$  & $0.5962  \pm  0.0104$  & $ 0.791  \pm   0.021$ \\
2.6  & $ 1.365  \pm   0.053$  & $0.6092  \pm  0.0131$  & $ 0.854  \pm   0.036$ \\
2.4  & $ 1.409  \pm   0.052$  & $0.6202  \pm  0.0100$  & $ 0.901  \pm   0.034$ \\
2.2  & $ 1.431  \pm   0.036$  & $0.6249  \pm  0.0105$  & $ 0.928  \pm   0.026$ \\
\hline 
\multicolumn{4}{l}{L80} \\ 
 \hline 
3.0  & $ 1.120  \pm   0.040$  & $0.6169  \pm  0.0185$  & $ 0.704  \pm   0.032$ \\
2.8  & $ 1.210  \pm   0.030$  & $0.6251  \pm  0.0115$  & $ 0.774  \pm   0.023$ \\
2.6  & $ 1.280  \pm   0.030$  & $0.6344  \pm  0.0117$  & $ 0.834  \pm   0.024$ \\
2.4  & $ 1.340  \pm   0.030$  & $0.6375  \pm  0.0078$  & $ 0.881  \pm   0.021$ \\
2.2  & $ 1.350  \pm   0.030$  & $0.6474  \pm  0.0120$  & $ 0.907  \pm   0.024$ \\
\hline 
\multicolumn{4}{l}{Planck} \\ 
 \hline 
3.0  & $ 1.072  \pm   0.059$  & $0.6462  \pm  0.0185$  & $ 0.657  \pm   0.045$ \\
2.8  & $ 1.155  \pm   0.065$  & $0.6573  \pm  0.0167$  & $ 0.723  \pm   0.049$ \\
2.6  & $ 1.254  \pm   0.044$  & $0.6601  \pm  0.0109$  & $ 0.791  \pm   0.034$ \\
2.4  & $ 1.290  \pm   0.074$  & $0.6784  \pm  0.0154$  & $ 0.840  \pm   0.056$ \\
2.2  & $ 1.316  \pm   0.057$  & $0.6751  \pm  0.0141$  & $ 0.858  \pm   0.044$ \\
\hline 


==> tables/table_Q2lliure_qpm8_par.tex <==
\begin{table}[!htbp]
 \adjustbox{width=1.2 \textwidth}{ 
  \begin{tabular}{c|*{6}c}
 z  &  $q_1$ & $q_2$  &  $k_p$  &  $k_v$  &  $a_v$  &  $b_v$ \\ 
  \hline 
  \hline 
  \multicolumn{7}{l}{Fiducial} \\ 
 \hline 
3.0  & $0.1042  \pm  0.1216$  & $ 0.444  \pm   0.093$  & $  10.1  \pm     0.5$  & $ 0.516  \pm   0.114$  & $ 0.248  \pm   0.072$  & $  1.66  \pm    0.02$ \\
2.8  & $0.0866  \pm  0.1101$  & $ 0.417  \pm   0.078$  & $   9.9  \pm     0.5$  & $ 0.493  \pm   0.087$  & $ 0.217  \pm   0.069$  & $  1.63  \pm    0.02$ \\
2.6  & $0.0687  \pm  0.1013$  & $ 0.390  \pm   0.063$  & $   9.6  \pm     0.5$  & $ 0.483  \pm   0.052$  & $ 0.190  \pm   0.056$  & $  1.61  \pm    0.02$ \\
2.4  & $0.0579  \pm  0.0853$  & $ 0.368  \pm   0.049$  & $   9.2  \pm     0.3$  & $ 0.480  \pm   0.028$  & $ 0.156  \pm   0.045$  & $  1.57  \pm    0.02$ \\
2.2  & $0.0902  \pm  0.0522$  & $ 0.316  \pm   0.027$  & $   8.9  \pm     0.3$  & $ 0.493  \pm   0.016$  & $ 0.145  \pm   0.031$  & $  1.54  \pm    0.01$ \\
\hline 
\multicolumn{7}{l}{R384C} \\ 
 \hline 
3.0  & $0.2073  \pm  0.2084$  & $ 0.320  \pm   0.159$  & $  11.2  \pm     1.0$  & $ 0.468  \pm   0.165$  & $ 0.208  \pm   0.120$  & $  1.57  \pm    0.01$ \\
2.8  & $0.2023  \pm  0.1325$  & $ 0.289  \pm   0.094$  & $  11.4  \pm     0.8$  & $ 0.462  \pm   0.111$  & $ 0.207  \pm   0.093$  & $  1.57  \pm    0.01$ \\
2.6  & $0.2036  \pm  0.0730$  & $ 0.267  \pm   0.041$  & $  11.2  \pm     0.4$  & $ 0.467  \pm   0.035$  & $ 0.198  \pm   0.042$  & $  1.57  \pm    0.01$ \\
2.4  & $0.2081  \pm  0.0832$  & $ 0.246  \pm   0.035$  & $  11.0  \pm     0.3$  & $ 0.475  \pm   0.019$  & $ 0.182  \pm   0.027$  & $  1.54  \pm    0.01$ \\
2.2  & $0.2335  \pm  0.0623$  & $ 0.213  \pm   0.023$  & $  10.8  \pm     0.2$  & $ 0.499  \pm   0.015$  & $ 0.181  \pm   0.019$  & $  1.51  \pm    0.01$ \\
\hline 
\multicolumn{7}{l}{L120} \\ 
 \hline 
3.0  & $0.5294  \pm  0.1152$  & $ 0.117  \pm   0.102$  & $  10.6  \pm     0.6$  & $ 0.684  \pm   0.196$  & $ 0.362  \pm   0.085$  & $  1.54  \pm    0.01$ \\
2.8  & $0.3989  \pm  0.1123$  & $ 0.190  \pm   0.087$  & $  10.5  \pm     0.6$  & $ 0.583  \pm   0.167$  & $ 0.290  \pm   0.076$  & $  1.55  \pm    0.01$ \\
2.6  & $0.3169  \pm  0.1050$  & $ 0.226  \pm   0.070$  & $  10.3  \pm     0.7$  & $ 0.529  \pm   0.118$  & $ 0.233  \pm   0.074$  & $  1.54  \pm    0.01$ \\
2.4  & $0.2644  \pm  0.0913$  & $ 0.241  \pm   0.060$  & $   9.9  \pm     0.6$  & $ 0.501  \pm   0.069$  & $ 0.183  \pm   0.065$  & $  1.53  \pm    0.01$ \\
2.2  & $0.2453  \pm  0.0867$  & $ 0.232  \pm   0.051$  & $   9.6  \pm     0.6$  & $ 0.497  \pm   0.046$  & $ 0.153  \pm   0.059$  & $  1.51  \pm    0.01$ \\
\hline 
\multicolumn{7}{l}{L80} \\ 
 \hline 
3.0  & $0.1440  \pm  0.2320$  & $ 0.430  \pm   0.202$  & $   8.9  \pm     0.8$  & $ 0.514  \pm   0.286$  & $ 0.212  \pm   0.158$  & $  1.61  \pm    0.01$ \\
2.8  & $0.1300  \pm  0.1330$  & $ 0.394  \pm   0.108$  & $   9.0  \pm     0.6$  & $ 0.490  \pm   0.108$  & $ 0.190  \pm   0.093$  & $  1.59  \pm    0.01$ \\
2.6  & $0.1170  \pm  0.1100$  & $ 0.367  \pm   0.080$  & $   8.9  \pm     0.5$  & $ 0.480  \pm   0.059$  & $ 0.167  \pm   0.071$  & $  1.56  \pm    0.01$ \\
2.4  & $0.1470  \pm  0.0820$  & $ 0.320  \pm   0.054$  & $   8.8  \pm     0.4$  & $ 0.493  \pm   0.041$  & $ 0.161  \pm   0.054$  & $  1.53  \pm    0.01$ \\
2.2  & $0.1200  \pm  0.0830$  & $ 0.308  \pm   0.047$  & $   8.5  \pm     0.4$  & $ 0.484  \pm   0.021$  & $ 0.123  \pm   0.050$  & $  1.50  \pm    0.01$ \\
\hline 
\multicolumn{7}{l}{Planck} \\ 
 \hline 
3.0  & $0.0004  \pm  0.2241$  & $ 0.787  \pm   0.220$  & $  11.8  \pm     1.2$  & $ 0.552  \pm   0.201$  & $ 0.178  \pm   0.108$  & $  1.64  \pm    0.03$ \\
2.8  & $-0.0168  \pm  0.1686$  & $ 0.711  \pm   0.143$  & $  12.0  \pm     1.0$  & $ 0.548  \pm   0.126$  & $ 0.203  \pm   0.073$  & $  1.65  \pm    0.03$ \\
2.6  & $0.0004  \pm  0.1241$  & $ 0.651  \pm   0.113$  & $  11.8  \pm     1.0$  & $ 0.545  \pm   0.115$  & $ 0.195  \pm   0.073$  & $  1.64  \pm    0.02$ \\
2.4  & $-0.0020  \pm  0.1108$  & $ 0.623  \pm   0.069$  & $  10.9  \pm     0.5$  & $ 0.517  \pm   0.027$  & $ 0.152  \pm   0.035$  & $  1.62  \pm    0.02$ \\
2.2  & $0.0405  \pm  0.0890$  & $ 0.534  \pm   0.049$  & $  10.6  \pm     0.3$  & $ 0.534  \pm   0.022$  & $ 0.139  \pm   0.029$  & $  1.60  \pm    0.01$ \\
\hline 
  \end{tabular}
 }
 \end{table}
 

==> tables/table_flx_apm7_par.tex <==
\begin{table}[!htbp]
 \adjustbox{width=1.2 \textwidth}{ 
  \begin{tabular}{c|*{6}c}
 z  &  $q_{1}$  &  $k_p\,[h/Mpc]$ &  $k_{v}^{a_v}\,[h/Mpc]^{a_v}$  &  $a_v$  &  $b_v$ &  $k_{na}$ \\ 
  \hline 
  \hline 
  \multicolumn{7}{l}{Fidu} \\ 
 \hline 
3.0  & $0.648  \pm  0.042$  & $13.1  \pm  0.42$  & $1.01  \pm  0.1$  & $0.627  \pm  0.033$  & $1.66  \pm  0.013$  & $4.09  \pm  0.04$ \\
2.8  & $0.644  \pm  0.037$  & $13.4  \pm  0.46$  & $0.979  \pm  0.091$  & $0.61  \pm  0.03$  & $1.64  \pm  0.013$  & $3.89  \pm  0.033$ \\
2.6  & $0.652  \pm  0.034$  & $13.6  \pm  0.47$  & $0.97  \pm  0.084$  & $0.59  \pm  0.028$  & $1.61  \pm  0.011$  & $3.65  \pm  0.036$ \\
2.4  & $0.666  \pm  0.03$  & $13.5  \pm  0.48$  & $0.963  \pm  0.076$  & $0.561  \pm  0.027$  & $1.58  \pm  0.01$  & $3.39  \pm  0.03$ \\
2.2  & $0.677  \pm  0.027$  & $13.3  \pm  0.53$  & $0.961  \pm  0.07$  & $0.533  \pm  0.025$  & $1.54  \pm  0.0097$  & $3.11  \pm  0.028$ \\
\hline 
\multicolumn{7}{l}{F_fixed} \\ 
 \hline 
3.0  & $0.71  \pm  0.041$  & $16  \pm  0.78$  & $1.19  \pm  0.11$  & $0.703  \pm  0.033$  & $1.66  \pm  0.021$  & $4.12  \pm  0.039$ \\
2.8  & $0.683  \pm  0.036$  & $14.7  \pm  0.66$  & $1.07  \pm  0.093$  & $0.644  \pm  0.029$  & $1.64  \pm  0.022$  & $3.88  \pm  0.037$ \\
2.6  & $0.652  \pm  0.033$  & $13.6  \pm  0.53$  & $0.97  \pm  0.083$  & $0.59  \pm  0.029$  & $1.61  \pm  0.02$  & $3.65  \pm  0.032$ \\
2.4  & $0.62  \pm  0.03$  & $12.5  \pm  0.45$  & $0.876  \pm  0.071$  & $0.53  \pm  0.027$  & $1.58  \pm  0.02$  & $3.43  \pm  0.034$ \\
2.2  & $0.585  \pm  0.028$  & $11.6  \pm  0.35$  & $0.793  \pm  0.064$  & $0.473  \pm  0.026$  & $1.56  \pm  0.019$  & $3.22  \pm  0.038$ \\
\hline 
\multicolumn{7}{l}{z_fixed} \\ 
 \hline 
0.696  & $0.585  \pm  0.034$  & $11.7  \pm  0.35$  & $0.811  \pm  0.074$  & $0.517  \pm  0.03$  & $1.62  \pm  0.022$  & $3.61  \pm  0.036$ \\
0.74  & $0.614  \pm  0.034$  & $12.5  \pm  0.42$  & $0.885  \pm  0.08$  & $0.555  \pm  0.029$  & $1.61  \pm  0.021$  & $3.65  \pm  0.039$ \\
0.781  & $0.652  \pm  0.034$  & $13.6  \pm  0.52$  & $0.969  \pm  0.085$  & $0.59  \pm  0.029$  & $1.61  \pm  0.022$  & $3.65  \pm  0.032$ \\
0.818  & $0.698  \pm  0.034$  & $14.8  \pm  0.69$  & $1.06  \pm  0.09$  & $0.62  \pm  0.029$  & $1.61  \pm  0.019$  & $3.6  \pm  0.026$ \\
0.8518  & $0.751  \pm  0.044$  & $16.4  \pm  1.1$  & $1.16  \pm  0.12$  & $0.646  \pm  0.035$  & $1.6  \pm  0.021$  & $3.52  \pm  0.026$ \\
\hline 
  \end{tabular}
 }
 \end{table}
 

==> tables/table_tests_apm7_bias.tex <==
\begin{table}[!htbp]
 \adjustbox{width=1.2 \textwidth}{ 
  \begin{tabular}{c|*{3}c}
 z  & $\beta$  &  $b_{\tau\delta}$  & $b_{\tau\eta}$   \\ 
  \hline 
  \hline 
  \multicolumn{4}{l}{Fidu} \\ 
 \hline 
3.0  & $1.21  \pm  0.049$  & $0.555  \pm  0.0086$  & $0.681  \pm  0.028$ \\
2.8  & $1.28  \pm  0.052$  & $0.558  \pm  0.0083$  & $0.733  \pm  0.03$ \\
2.6  & $1.34  \pm  0.055$  & $0.559  \pm  0.0084$  & $0.771  \pm  0.032$ \\
2.4  & $1.39  \pm  0.056$  & $0.557  \pm  0.008$  & $0.796  \pm  0.032$ \\
2.2  & $1.4  \pm  0.061$  & $0.554  \pm  0.0079$  & $0.807  \pm  0.034$ \\
\hline 
\multicolumn{4}{l}{P1024} \\ 
 \hline 
3.0  & $1.21  \pm  0.05$  & $0.557  \pm  0.098$  & $0.684  \pm  0.12$ \\
2.8  & $1.28  \pm  0.052$  & $0.56  \pm  0.0084$  & $0.735  \pm  0.03$ \\
2.6  & $1.34  \pm  0.056$  & $0.561  \pm  0.0084$  & $0.772  \pm  0.033$ \\
2.4  & $1.38  \pm  0.059$  & $0.56  \pm  0.0082$  & $0.797  \pm  0.034$ \\
2.2  & $1.4  \pm  0.061$  & $0.556  \pm  0.008$  & $0.809  \pm  0.035$ \\
\hline 
\multicolumn{4}{l}{L120} \\ 
 \hline 
3.0  & $1.19  \pm  0.039$  & $0.571  \pm  0.0057$  & $0.695  \pm  0.023$ \\
2.8  & $1.28  \pm  0.04$  & $0.577  \pm  0.0058$  & $0.757  \pm  0.024$ \\
2.6  & $1.36  \pm  0.042$  & $0.581  \pm  0.0057$  & $0.808  \pm  0.025$ \\
2.4  & $1.41  \pm  0.042$  & $0.582  \pm  0.0059$  & $0.847  \pm  0.025$ \\
2.2  & $1.44  \pm  0.044$  & $0.579  \pm  0.0051$  & $0.867  \pm  0.025$ \\
\hline 
\multicolumn{4}{l}{R384C} \\ 
 \hline 
3.0  & $1.21  \pm  0.06$  & $0.566  \pm  0.0094$  & $0.698  \pm  0.035$ \\
2.8  & $1.29  \pm  0.06$  & $0.571  \pm  0.0097$  & $0.754  \pm  0.036$ \\
2.6  & $1.36  \pm  0.06$  & $0.573  \pm  0.0086$  & $0.8  \pm  0.035$ \\
2.4  & $1.42  \pm  0.05$  & $0.571  \pm  0.0065$  & $0.837  \pm  0.029$ \\
2.2  & $1.46  \pm  0.064$  & $0.559  \pm  0.0085$  & $0.844  \pm  0.037$ \\
\hline 
\multicolumn{4}{l}{R384} \\ 
 \hline 
3.0  & $1.18  \pm  0.06$  & $0.571  \pm  0.01$  & $0.687  \pm  0.036$ \\
2.8  & $1.27  \pm  0.06$  & $0.574  \pm  0.0096$  & $0.746  \pm  0.036$ \\
2.6  & $1.33  \pm  0.06$  & $0.576  \pm  0.0086$  & $0.787  \pm  0.035$ \\
2.4  & $1.38  \pm  0.07$  & $0.576  \pm  0.0087$  & $0.82  \pm  0.041$ \\
2.2  & $1.42  \pm  0.07$  & $0.57  \pm  0.0099$  & $0.841  \pm  0.041$ \\
\hline 
\multicolumn{4}{l}{R640} \\ 
 \hline 
3.0  & $1.25  \pm  0.052$  & $0.541  \pm  0.095$  & $0.69  \pm  0.12$ \\
2.8  & $1.32  \pm  0.054$  & $0.546  \pm  0.0085$  & $0.735  \pm  0.031$ \\
2.6  & $1.36  \pm  0.054$  & $0.548  \pm  0.0082$  & $0.768  \pm  0.031$ \\
2.4  & $1.4  \pm  0.056$  & $0.549  \pm  0.0079$  & $0.791  \pm  0.032$ \\
2.2  & $1.42  \pm  0.061$  & $0.546  \pm  0.0085$  & $0.805  \pm  0.034$ \\
\hline 


==> tables/table_tests_apm7_par.tex <==
\begin{table}[!htbp]
 \adjustbox{width=1.2 \textwidth}{ 
  \begin{tabular}{c|*{6}c}
 z  &  $q_{1}$  &  $k_p\,[h/Mpc]$ &  $k_{v}^{a_v}\,[h/Mpc]^{a_v}$  &  $a_v$  &  $b_v$ &  $k_{\mu}$ \\ 
  \hline 
  \hline 
  \multicolumn{7}{l}{Fidu} \\ 
 \hline 
3.0  & $0.648  \pm  0.042$  & $13.1  \pm  0.42$  & $1.01  \pm  0.1$  & $0.627  \pm  0.033$  & $1.66  \pm  0.013$  & $4.09  \pm  0.04$ \\
2.8  & $0.644  \pm  0.037$  & $13.4  \pm  0.46$  & $0.979  \pm  0.091$  & $0.61  \pm  0.03$  & $1.64  \pm  0.013$  & $3.89  \pm  0.033$ \\
2.6  & $0.652  \pm  0.034$  & $13.6  \pm  0.47$  & $0.97  \pm  0.084$  & $0.59  \pm  0.028$  & $1.61  \pm  0.011$  & $3.65  \pm  0.036$ \\
2.4  & $0.666  \pm  0.03$  & $13.5  \pm  0.48$  & $0.963  \pm  0.076$  & $0.561  \pm  0.027$  & $1.58  \pm  0.01$  & $3.39  \pm  0.03$ \\
2.2  & $0.677  \pm  0.027$  & $13.3  \pm  0.53$  & $0.961  \pm  0.07$  & $0.533  \pm  0.025$  & $1.54  \pm  0.0097$  & $3.11  \pm  0.028$ \\
\hline 
\multicolumn{7}{l}{P1024} \\ 
 \hline 
3.0  & $0.644  \pm  0.042$  & $13.2  \pm  0.45$  & $0.997  \pm  0.1$  & $0.634  \pm  0.032$  & $1.66  \pm  0.024$  & $4.09  \pm  0.04$ \\
2.8  & $0.642  \pm  0.037$  & $13.5  \pm  0.56$  & $0.973  \pm  0.091$  & $0.617  \pm  0.03$  & $1.63  \pm  0.022$  & $3.89  \pm  0.033$ \\
2.6  & $0.65  \pm  0.035$  & $13.7  \pm  0.51$  & $0.964  \pm  0.084$  & $0.597  \pm  0.029$  & $1.6  \pm  0.02$  & $3.65  \pm  0.036$ \\
2.4  & $0.665  \pm  0.031$  & $13.6  \pm  0.53$  & $0.959  \pm  0.075$  & $0.567  \pm  0.026$  & $1.57  \pm  0.015$  & $3.39  \pm  0.03$ \\
2.2  & $0.679  \pm  0.028$  & $13.4  \pm  0.5$  & $0.956  \pm  0.069$  & $0.537  \pm  0.025$  & $1.53  \pm  0.014$  & $3.11  \pm  0.028$ \\
\hline 
\multicolumn{7}{l}{L120} \\ 
 \hline 
3.0  & $0.661  \pm  0.032$  & $11.3  \pm  0.24$  & $0.803  \pm  0.064$  & $0.46  \pm  0.026$  & $1.55  \pm  0.01$  & $4.01  \pm  0.034$ \\
2.8  & $0.635  \pm  0.028$  & $12  \pm  0.29$  & $0.782  \pm  0.057$  & $0.471  \pm  0.024$  & $1.56  \pm  0.0099$  & $3.8  \pm  0.031$ \\
2.6  & $0.626  \pm  0.026$  & $12.7  \pm  0.36$  & $0.772  \pm  0.053$  & $0.469  \pm  0.023$  & $1.56  \pm  0.0096$  & $3.56  \pm  0.02$ \\
2.4  & $0.633  \pm  0.023$  & $13.2  \pm  0.4$  & $0.771  \pm  0.048$  & $0.456  \pm  0.021$  & $1.54  \pm  0.011$  & $3.29  \pm  0.018$ \\
2.2  & $0.643  \pm  0.02$  & $13.5  \pm  0.56$  & $0.778  \pm  0.046$  & $0.439  \pm  0.02$  & $1.52  \pm  0.011$  & $3  \pm  0.015$ \\
\hline 
\multicolumn{7}{l}{R384C} \\ 
 \hline 
3.0  & $0.592  \pm  0.051$  & $14  \pm  0.6$  & $0.786  \pm  0.1$  & $0.504  \pm  0.042$  & $1.57  \pm  0.01$  & $4.15  \pm  0.05$ \\
2.8  & $0.578  \pm  0.045$  & $14.9  \pm  0.8$  & $0.774  \pm  0.095$  & $0.509  \pm  0.038$  & $1.58  \pm  0.01$  & $3.92  \pm  0.047$ \\
2.6  & $0.584  \pm  0.039$  & $15.5  \pm  0.9$  & $0.773  \pm  0.083$  & $0.5  \pm  0.036$  & $1.58  \pm  0.02$  & $3.67  \pm  0.039$ \\
2.4  & $0.602  \pm  0.032$  & $15.9  \pm  1.1$  & $0.778  \pm  0.064$  & $0.478  \pm  0.028$  & $1.55  \pm  0.01$  & $3.4  \pm  0.034$ \\
2.2  & $0.644  \pm  0.027$  & $15.4  \pm  0.81$  & $0.822  \pm  0.06$  & $0.458  \pm  0.024$  & $1.52  \pm  0.017$  & $3.12  \pm  0.032$ \\
\hline 
\multicolumn{7}{l}{R384} \\ 
 \hline 
3.0  & $0.586  \pm  0.051$  & $12.9  \pm  0.5$  & $0.921  \pm  0.12$  & $0.617  \pm  0.041$  & $1.66  \pm  0.02$  & $4.13  \pm  0.046$ \\
2.8  & $0.584  \pm  0.043$  & $13.3  \pm  0.5$  & $0.894  \pm  0.1$  & $0.6  \pm  0.038$  & $1.64  \pm  0.02$  & $3.93  \pm  0.047$ \\
2.6  & $0.594  \pm  0.041$  & $13.6  \pm  0.6$  & $0.885  \pm  0.097$  & $0.578  \pm  0.037$  & $1.61  \pm  0.01$  & $3.68  \pm  0.038$ \\
2.4  & $0.612  \pm  0.038$  & $13.7  \pm  0.7$  & $0.877  \pm  0.089$  & $0.547  \pm  0.034$  & $1.58  \pm  0.01$  & $3.42  \pm  0.031$ \\
2.2  & $0.634  \pm  0.03$  & $13.5  \pm  0.6$  & $0.88  \pm  0.079$  & $0.514  \pm  0.032$  & $1.54  \pm  0.01$  & $3.13  \pm  0.032$ \\
\hline 
\multicolumn{7}{l}{R640} \\ 
 \hline 
3.0  & $0.642  \pm  0.042$  & $14.9  \pm  0.82$  & $1.02  \pm  0.11$  & $0.651  \pm  0.034$  & $1.71  \pm  0.025$  & $4.14  \pm  0.043$ \\
2.8  & $0.633  \pm  0.038$  & $15.1  \pm  0.7$  & $0.998  \pm  0.094$  & $0.636  \pm  0.03$  & $1.68  \pm  0.022$  & $3.95  \pm  0.041$ \\
2.6  & $0.636  \pm  0.034$  & $15.1  \pm  0.69$  & $0.984  \pm  0.085$  & $0.614  \pm  0.028$  & $1.65  \pm  0.021$  & $3.71  \pm  0.04$ \\
2.4  & $0.645  \pm  0.03$  & $14.8  \pm  0.63$  & $0.969  \pm  0.077$  & $0.582  \pm  0.027$  & $1.61  \pm  0.013$  & $3.45  \pm  0.019$ \\
2.2  & $0.656  \pm  0.027$  & $14.4  \pm  0.67$  & $0.95  \pm  0.071$  & $0.543  \pm  0.026$  & $1.57  \pm  0.017$  & $3.16  \pm  0.032$ \\
\hline 
  \end{tabular}
 }
 \end{table}
 
